Balanced Data, Imbalanced Spectra: Unveiling Class Disparities with Spectral Imbalance

Classification models are expected to perform equally well for different classes, yet in practice, there are often large gaps in their performance. This issue of class bias is widely studied in cases of datasets with sample imbalance, but is relatively overlooked in balanced datasets. In this work, we introduce the concept of spectral imbalance in features as a potential source for class disparities and study the connections between spectral imbalance and class bias in both theory and practice. To build the connection between spectral imbalance and class gap, we develop a theoretical framework for studying class disparities and derive exact expressions for the per-class error in a high-dimensional mixture model setting. We then study this phenomenon in 11 different state-of-the-art pretrained encoders and show how our proposed framework can be used to compare the quality of encoders, as well as evaluate and combine data augmentation strategies to mitigate the issue. Our work sheds light on the class-dependent effects of learning, and provides new insights into how state-of-the-art pretrained features may have unknown biases that can be diagnosed through their spectra.

==> symbols.tex <==
% Define all the modified symbols one could think of.
% Adapted from https://tex.stackexchange.com/questions/477180/loop-over-greek-letters-with-pgffor

% Usage:
% Uppercase Roman: \blA = bold uppercase A. \opA = operator, \scrA = script, \Ahat = hat, \Abr = bar, \Atl = tilde
% Lowercase Roman: \bla, etc. No operator or script.
% Greek: same as Roman with \blGamma, \alphahat, \Xitl, etc.


%\newcommand{\op}[1]{\operatorname{\symcal{#1}}}
%\newcommand{\opbar}[1]{\operatorname{\overline{\symcal{#1}}}}
\newcommand{\scrbar}[1]{\overline{\mathcal{#1}}}

\ExplSyntaxOn

\cs_new_protected:Nn \bamboo_define:nnnnnN
% #1 = name, #2 = argument, #3 = prefix, #4 = suffix, #5 = decoration, #6 = how to interpret decoration
{
	\cs_new_protected:cpx { #3 #1 #4 } { \exp_not:N #5{#6{#2}} }
}

\int_step_inline:nnn { `A } { `Z }
{
	% Bold
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ bl }
	{ }
	{ \mymathbold }
	\use:n
	
%	% Operator
%	\bamboo_define:nnnnnN
%	{ \char_generate:nn { #1 } { 11 } }
%	{ \char_generate:nn { #1 } { 11 } }
%	{ op }
%	{ }
%	{ \op }
%	\use:n
	
	% Script
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ scr }
	{ }
	{ \mathcal }
	\use:n
	
	% Hat
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ hat }
	{ \widehat }
	\use:n
	
	% Bar
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ br }
	{ \overline }
	\use:n
	
	% Tilde
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ tl }
	{ \widetilde }
	\use:n
	
	% Script with bar
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ scr }
	{ br }
	{ \scrbar }
	\use:n
}
\int_step_inline:nnn { `a } { `z }
{
	% Bold
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ bl }
	{ }
	{ \mymathbold }
	\use:n
	
	% Hat
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ hat }
	{ \hat }
	\use:n
	
	% Bar
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ br }
	{ \bar }
	\use:n
	
	% Tilde
	\bamboo_define:nnnnnN
	{ \char_generate:nn { #1 } { 11 } }
	{ \char_generate:nn { #1 } { 11 } }
	{ }
	{ tl }
	{ \tilde }
	\use:n                            % just the argument
}
\clist_map_inline:nn
{
	Gamma,Delta,Theta,Lambda,Xi,Pi,Sigma,Phi,Psi,Omega
}
{
	% Bold
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ bl }
	{ }
	{ \mymathbold }
	\use:c
	
	% Operator
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ op }
	{ }
	{ \op }
	\use:c
	
	% Script
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ scr }
	{ }
	{ \mathcal }
	\use:c
	
	% Hat
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ hat }
	{ \widehat }
	\use:c
	
	% Bar
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ br }
	{ \overline }
	\use:c
	
	% Tilde
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ tl }
	{ \widetilde }
	\use:c
}
\clist_map_inline:nn
{
	alpha,beta,gamma,delta,epsilon,zeta,eta,theta,iota,kappa,
	lambda,mu,nu,xi,pi,rho,sigma,tau,phi,chi,psi,omega
}
{
	% Bold
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ bl }
	{ }
	{ \mymathbold }
	\use:c
	
	% Hat
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ hat }
	{ \hat }
	\use:c
	
	% Bar
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ br }
	{ \bar }
	\use:c
	
	% Tilde
	\bamboo_define:nnnnnN
	{ #1 }
	{ #1 }
	{ }
	{ tl }
	{ \tilde }
	\use:c
}

\ExplSyntaxOff

==> tables/hyser-results.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{cc|cc|cc|ccc|c}
& & \multicolumn{2}{c}{Action recognition} & \multicolumn{2}{c}{DoF} &  \multicolumn{3}{c}{Force prediction} & \\
& Model & Dynamic & Maintenance & 1-DoF & N-DoF & MVC & DoF & random & Avg. \\

\hline\hline

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Clf}}}
& Rand. Init. & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& Linear Probing & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& EIT \cite{liu2022seeing} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\

\hline

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{Reg}}}
& Rand. Init. & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& Linear Probing & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
& EIT \cite{liu2022seeing} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
\hline\hline
\end{tabular}
\end{center}
\caption{{\em Results on Hyser multitask.}~ ABC
}
\label{table:hyser}
\end{table*}

==> tables/spectral_table.tex <==
\begin{table}[t]
\caption{\footnotesize{Examining spectral imbalance on different pretrained encoders. The correlation between across-class accuracies and the across-class spectra (Max-Corr), gap in accuracies across classes (Acc Gap) and spectral imbalance rate (SI) are calculated.}
\color{red}{SI rate and Acc Gap are already in Fig.1. Should we put them here again? I feel it repetitive but also too far away.}
}
\label{sample-table}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Model & Max Corr. & PL Corr. & SI rate \\
\midrule
Densenet & 0.6677 & 0.6636  & - \\
EfficientNet-B1 & 0.7599 & 0.7476  & - \\
EfficientNet-B3 & 0.7505 & 0.7210  & - \\
Resnet-18    & 0.6229 & 0.5649 & - \\
Resnet-50    & 0.6293 & 0.6270  & - \\
Resnet-101   & 0.6560 & 0.6454  & - \\
VIT-S      & 0.6891 & 0.6783  & - \\
VIT-B      & 0.6536 & 0.6531  & - \\
MLPMixer   & 0.7785 & 0.7715  & - \\
Poolformer-S24  & 0.6961 & 0.6755  & - \\
Poolformer-S36  & 0.7062 & 0.6904  & - \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}



==> texts/experiments_removed.tex <==
\begin{figure}[t!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{imgs/da_empirical_placeholder.png}}
\caption{Data augmentation empirical results.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Data augmentations experimental results}
% \label{sec:method}

When having data augmentation $T$ which creates augmented version of the data $T(x)$, the estimation becomes:
\begin{equation}
\Sigma_C^{k}\left(\mathbf{f}_\theta\right)=\frac{1}{k N_C} \sum_{i=1}^{k N_C} \mathbf{f}_\theta\left(T(x_i)\right) \mathbf{f}_\theta\left(T(x_i)\right)^T    
\end{equation}
where $k$ means for each sample, the data augmentation is applied $k$ times.

% \subsection{How many data augmentations are applied}

We first study how the eigenspectrum would change when applying the data augmentation many times. Observation, it converges when $k$ is large enough, which is the common setting in practice.
Interestingly, we observe that the data augmentation policy people apply in reality gives better eigenspectrum (lower values.)


% \subsection{Judging data augmentation from the perspective of eigenspectrum}


We further study the effect of data augmentation policies used in natural images. Specifically, the data augmentation policies we study include random cropping, color jittering, flipping of images, and etc.
When changing some parameter of the data augmentation; we observe how its eigenspectrum is changed, and this can guide us to select the best data augmentation policy for that class.




%\begin{table}[t]
%\caption{\footnotesize{Performance on Imagenet-C. The correlation between across-class accuracies and the across-class spectra (Max-Corr), gap in accuracies across classes (Acc Gap) and spectral imbalance rate (SI) are computed for all of the pretrained encoders.}}
%\label{sample-table}
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lcccr}
%\toprule
% Model & Max Corr. & Acc. Gap & SI rate \\
%\midrule
%ResNet    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& - \\
%ViT & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& -\\
%EffNet    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& - \\
%D    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&    -     \\
%E     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& - \\
%Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& - \\
%Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&  -       \\
%Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& - \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table}

% \section{The class-dependent effect of augmentations}
% \label{sec:method}

% When having data augmentation $T$ which creates augmented version of the data $T(x)$, the estimation becomes:
% \begin{equation}
% \Sigma_C^{k}\left(\mathbf{f}_\theta\right)=\frac{1}{k N_C} \sum_{i=1}^{k N_C} \mathbf{f}_\theta\left(T(x_i)\right) \mathbf{f}_\theta\left(T(x_i)\right)^T    
% \end{equation}
% where $k$ means for each sample, the data augmentation is applied $k$ times.

% \subsection{How many data augmentations are applied}

% We first study how the eigenspectrum would change when applying the data augmentation many times. Observation, it converges when $k$ is large enough, which is the common setting in practice.
% Interestingly, we observe that the data augmentation policy people apply in reality gives better eigenspectrum (lower values.)


% \subsection{Judging data augmentation from the perspective of eigenspectrum}


% We further study the effect of data augmentation policies used in natural images. Specifically, the data augmentation policies we study include random cropping, color jittering, flipping of images, and etc.
% When changing some parameter of the data augmentation; we observe how its eigenspectrum is changed, and this can guide us to select the best data augmentation policy for that class.





%\begin{table}[h!]
%\caption{\footnotesize{Performance on Resnet (or XX) for different augmentations.}}
%\label{sample-table}
%\begin{center} \begin{small}
% \begin{sc}
%\begin{tabular}{lcccr}
%\toprule
%Model & Max Corr. & Acc. Gap & SI rate \\
%\midrule
%ResNet    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& - \\
%ViT & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& -\\
%EffNet    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& - \\
%D    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&    -     \\
%E     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& - \\
%Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& - \\
%Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&  -       \\
%Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& - \\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small} \end{center}
%\vskip -0.1in
%\end{table}



% \subsection{Latent space augmentation with Gaussian noise injection and random removing of latent features}

% Following the theoretical results, and inspired by research works that discover latent space augmentation based on Gaussian noise gives impressive improvement of performance (cite), we investigate if there exists systematic ways to perform latent space augmentation, how they could re-balance the spectral properties, and how they would influence class-wise performance in the studied datasets.

% \paragraph{Adding simple class-dependent Gaussian noise}

% This closes the class gap, yet does not systematically improve performance by a lot.

% \paragraph{Adding noise based on estimated eigenvectors}

% This does improve both performance and class bias I believe, but by a small margin and is very very slow, even on cifar10.

% \paragraph{Random masking}

% Didn't do it yet. Need to do this!

% \subsection{Analysis}


% \subsection{Class-dependent generalization of DA}
% Effect of aERM on generalization. Describe ridge regression equivalence and spectrum modifying effect. Shows that DA effects spectrum, but what are the implications for class gap?
% \paragraph{Theorem 2} Asymptotic prediction for per-class error with aERM.

% \begin{theorem}[Per-class generalization of DA]\label{thm:class_dep_da}
% Let $\TT$ and $\tSIG_y$ be the augmentation-modified target signal and covariances, respectively, and let $\tilde{\Q} = [\tSIG_{y_1}^{1/2} \z_1, \dots, \tSIG_{y_n}^{1/2} \z_n]^\top$, $\A = n \I + \tilde{\Q}\tilde{\Q}^\top$, and $\tSIG = \frac{\tSIG_1 + \tSIG_{-1}}{2}$. Choose $k\leq n$ so that the condition number of $\A_k$ is bounded by $L$ with probability $1-\delta$. Furthermore, Let $\kappa$ be the condition number of $\mathbb{E}_\x \text{Cov}_G(\X)$ and $\tilde{\kappa}$ be the condition number of $\tilde{\SIG}_y$. 

% Then, if $\tilde{\kappa}^{1/2} \Delta \lesssim 1$ and $\frac{\operatorname{tr}(\tSIG)}{n} \geq CL \max \left\{1, \|\tSIG\|_{2}, \|\TT\|_{\tSIG}\right\}$, the class dependent POE of the aERM estimator is bounded with probability at least $1-\delta-n^{-1}$ by 
% \[
%     %\text{POE}(\HT | y) \leq  
%     (\textcolor{red}{\text{EM}}) \exp\left(\frac{-C\|\TT\|_2^4}{\|\TT\|_{\tSIG_y}^2+ \tilde{E}_y\left(\|\tilde{\T}^*_{1:k}\|_{\tSIG_{1:k}^{-1}}^2\tilde{\lambda}^2_{k+1}\rho_{k}^2(\tSIG;n)+ \widetilde{T}_1)\right)}\right).
% \]
% Here, $\tilde{E}_y := \|\tSIG_y\tSIG^{-1}\|$, $\widetilde{T}_1 = \Vert \TT_{k+1:p}\Vert_{\tSIG_{k+1:p}}^2 + (\operatorname{tr}{\tSIG})^2 (\frac{k}{n^3}+\frac{1}{n R_k(\tSIG;n)}$ and the error multiplier \textcolor{red}{\text{EM}} is specified as 
% \[
% \textcolor{red}{\text{EM}} = \exp\left(\frac{C\kappa^{\frac{1}{2}}\Delta \Vert \TS \Vert_2^2 \Vert \BT \Vert_2^2}{\Vert \BT \Vert_{\SIG_y}^2} \right).
% \]
% \end{theorem}

% Comparing Theorem \ref{thm:class_dep_ridge} and \ref{thm:class_dep_da}, we can see that the generalization error of the aERM estimator is, up to the approximation term $\textcolor{red}{\text{EM}}$, equivalent to the POE of a ridge estimator for which the data covariance is $\tSIG_y$, the true signal is $\TT$, and the ridge parameter is $\lambda = n$. 

% \subsection{Training with class-specific augmentations}
% We can also extend our analysis framework to the case where training data is augmented differently for each class. Specifically, suppose augmentations are applied independently for each training sample, where $g_i \sim \mathcal{G}_y$ if $y_i = y$. For simplicity, suppose both augmentation distributions are unbiased (i.e. $\mathbb{E}_{\mathcal{G}_y} g(x) = x$). Then the aERM objective is given by
% $\E_G[\|G(\X)\T-\y)\|_2^2] = \E_G[\|\left(G(\X)-\mu(\X)\right)\T+\mu(\X)\T -\y)\|_2^2]  = \|\X\T - \y\|_2^2 + \|\T\|_{n\R}^2,
% $
% where $
% \R := \frac{1}{n} \sum_{i=1}^n \text{Cov}_{g_i}(x_i)$.

% Let $\HT = (\X^\top \X + n\R)^{-1} \X^\top \y$ be the solution to the above objective, and let $\BT = (\X^\top \X + n\bar{\R})^{-1} \X^\top \y$, where $\bar{\R} = \mathbb{E}_{\x} \R = (\mathbb{E}_{\x}[\text{Cov}_{\mathcal{G}_1}(\x) | y=1] + \mathbb{E}_{\x}[\text{Cov}_{\mathcal{G}_{-1}}(\x) | y=-1])/2.$

% Via a similar argument as above, we can write 
% \begin{align*}
% \text{POE}(\BT|y) &\leq  \exp\left(\frac{-C (\hat{\theta}_r^\top \tilde{\theta}^*)^2}{\Vert \hat{\theta}_r \Vert_{\tilde{\SIG}_y}^2}\right),
% \end{align*}
% where $\hat{\theta}_r$ is a ridge estimator with parameter $\lambda = n$, data $\tilde{\X} = \X \bar{\R}^{-1/2}$, true signal $\tilde{\theta}^* = \bar{\R}^{-1/2} \theta^*$, and $\tilde{\SIG}_y = \bar{\R}^{-1/2} \SIG_y \bar{\R}^{-1/2}$. This can in turn be bounded by applying Theorem \ref{thm:class_dep_ridge}. Finally, the approximation error term can be handled identically to in Lemma \ref{lem:appx}, where $\kappa$ is the condition number of $\bar{\R}$ and $\tilde{\kappa}$ be the condition number of $\tilde{\SIG}_y$.


% \begin{figure}[t!]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{imgs/da_empirical_placeholder.png}}
% \caption{Data augmentation empirical results.}
% \label{icml-historical}
% \end{center}
% \vskip -0.2in
% \end{figure}


% \subsection{Case study: Using DA to improve class gap}
% Adding a single pre-computed Gaussian noise augmentation can help reduce class gap, but there is a tradeoff with class accuracy. Add theorem
% \subsection{Empirical results in GMM: Predicting the per-class performance and class gap}

% Simulations of linear classifier in the GMM setting to show that the theoretical predictions are accurate. 
% Add here: Figure showing (i) measure of spectral gap vs class gap (predicted/simulated values), (ii) predictions of aERM with random mask, (iii -  if possible?) example of class-specific, pre-computed noise improving class gap (oracle and non-oracle cases)




==> texts/intro.tex <==
\section{Introduction}

When training machine learning models for classification, we want them to give good accuracy on all classes. 
However, it is more challenging to perform well on some classes and it is easy to on others, and this is the problem of class bias. 
Class bias is a severe problem, it leads to not only worse general performance, but also possible societal bias. 

% Machine learning models are often optimized to maximize the average accuracy across all classes. However, models trained using such approaches can generate problematic pre-trained features as they tend to treat all classes equally, even if some classes are inherently more difficult to classify. This can cause a severe issue of \textit{class bias}, which is accuracy differences within classes, which cause the model to generalize differently for different classes and it leads to catastrophic failures in certain cases.

% In modern applications where data augmentations are frequently performed, this class-dependent bias is even further amplified, with some classes improving and others having catastrophic failures under even mild augmentations.

\begin{figure}[t!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{imgs/overview_fig_SI.png}}
\caption{{\em Overview.} (A) In this work, we present the concept of spectrum imbalance, which connect class-wise performance with the imbalance of conditional eigenspectrum. (B) We show the Spectrum variation score of pre-trained networks closely associates with their class bias in terms of prediction accuracy.}
\label{fig:motivate}
\end{center}
\vskip -0.2in
\end{figure}


One source of such imbalance is due to the amount of number of samples per class, and that is vastly studied in the context of class-imbalanced learning (e.g. one of its famous and challenging form is long-tail recognition tasks).
% Current analysis of the generalization and class-dependent bias in machine learning has mainly focused on imbalance in terms of the number of samples per class. [Long-tail recognition literatures] 
While these are important issues to consider, one problem that people often neglect is that even in balanced dataset (e.g. ImageNet), the class bias is still strong and exist in large scale.
% there are many other ways in which learning can be imbalanced or unfair across classes.
This is a more valuable problem in the age of foundation models, because there are so many more data.
To address this gap in our understanding, we need new theory that will allow us to understand the class bias that is not relevant to the amount of samples.

% However, the amount of sample is not the only source of imbalance. Even when the amount of samples are the same, some classes are inherently more difficult to classify.

In this work, we introduce a new framework for analyzing class-dependent generalization, with a focus on a form of imbalance across classes that we refer to as \textit{spectral imbalance}. 
Spectral imbalance refers to situations where the distribution of features across different classes is significantly different, with some classes having large variance along certain directions and others having more restricted or clustered features. We show how such spectral imbalances can lead to poor generalization performance for certain classes, even when the number of samples in each class is equal. We provide a comprehensive analysis of class-dependent generalization using our framework, and derive bounds that depend on class-dependent spectral quantities. Furthermore, we demonstrate how our framework can be used to study the impact of different types of augmentations on per-class generalization, providing new insights into the effects of data augmentation on spectral imbalance.

After introducing our theory, we study pre-trained features of large-scale models, and observe that class bias is strongly correlated with the spectral properties of datasets in reality, aligning with the theory results.
We show such phenomena are consistently observed in reality, and can be used to predict the class performance (and imbalance between different classes) without ever training a linear layer. 
%We observe that data augmentation in reality can correct such imbalances, and thus improve class bias.
%Finally, we investigate if it is possible to design augmentations, or correct the existing data augmentations, in order to produce better pre-trained features for better training of the classifier.
Through the empirical study, we highlight the importance of spectral imbalance in reality, and provide ways to design better augmentations that improve overall performance and class gap.

%\begin{figure}[t]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{imgs/overview_placeholder.png}}
%\caption{An image showing how class-wise accuracy is correlated to spectrum property for many classes, with Pearson correlation displayed on right top corner. Would it look bad or something?}
%\label{fig:overview}
%\end{center}
%\vskip -0.2in
%\end{figure}


Major contributions are:
\begin{itemize}
\itemsep0em
    \item We derive \textit{exact} theoretical expressions for the per-class generalization in a high-dimensional mixture-model setting. The resultant predictions demonstrate the effect of spectral imbalance on the per-class performance gap. 
    \item Empirically, we show that similar phenomena holds in pretrained features of many pre-trained models across many different datasets,  making the spectral property a good evaluation metric on itself to predict the worst performing classes and the amount of ``imbalance'' between different classes.
    \item We study the effect of data augmentation under this spectral imbalance framework, and provide possible ways to use data sugmentation to improve class bias and generate more ``balanced'' pre-trained features.
\end{itemize}


==> texts/intro_v2.tex <==
\section{Introduction}
% class bias exists
One core objective of machine learning is building robust and balanced classification models that can provide good performance irrespective of the class in which the data lies. In practice, however, 
models are often biased towards better performance on some classes of the data. 
This is particularly relevant in the age of foundation and pretrained models, where some underlying biases in the features may exist that will impact some classes more than others.
% class bias v.s. group bias --> sample imbalance?


% class gap has been studied but its not enough
Most studies and approaches for dealing with class imbalance have focused on \textit{sample imbalance}, or the fact that different classes often have different number of samples \cite{zhang2023deep}. In this case, reweighting the loss or rebalancing the dataset through augmentation or class weights can be used to rebalance the numbers of samples \cite{ren2020balanced,zhu2022balanced}. 
However, 
even in a balanced 
dataset (e.g. ImageNet), there still can be significant gaps in performance across classes, even for state-of-the-art encoders \cite{balestriero2022effects}. 
The presence of \emph{class disparity} even on balanced datasets is overlooked in the empirical literature, and why it occurs is a significantly more subtle question.
Can we understand the source of class disparities here, and how to characterize it in different encoders?


In this work, we study class-dependent generalization, and show the prevalence of imbalance across classes in the representation space that we refer to as \textit{spectral imbalance}. Informally, spectral imbalance refers to situations where the distribution of features across different classes is significantly different, with some classes having large variance along certain directions and others having more restricted or clustered features. 
We show how such imbalances can lead to poor generalization performance for certain classes, even when the number of training samples per class is identical. 

First, we develop a theoretical framework for studying this phenomenon and dig deeper into the distinct ways in which spectral imbalance may impact class gap.  In particular, we derive \textit{exact asymptotic expressions} for the class-wise error and class gap in a Gaussian mixture model with class-specific covariances. 
We use these expressions to uncover different quantitative manifestations of spectral imbalance and characterize their consequences for the class gap.
% By allowing for different covariances to model the different spectral components within the data, we can use this analysis to study a number of different ways in which spectral imbalance can be understood. We reveal that, in particular, XX type of imbalance in the spectra has the most severe impact on class gap, and that UU happens in these models.

% We provide a comprehensive analysis of class-dependent generalization using our framework, and derive bounds that depend on class-dependent spectral quantities. Furthermore, we demonstrate how our framework can be used to study the impact of different types of augmentations on per-class generalization, providing new insights into the effects of data augmentation on spectral imbalance.

To understand how spectral imbalance and class bias may manifest in empirical experiments,
% pre-trained features of large-scale models, 
we 
%further develop an empirical framework to model and study spectral imbalance in the representation space
study spectral differences in the representation space of 11 state-of-the-art pre-trained encoders (using 6 distinct styles of architecture) on ImageNet. % across a wide range of Resnet and transformer encoders. 
Across the board, we observe that class disparity is strongly correlated with the spectral imbalance of the representation space. 
Furthermore, we use a ``spectral imbalance" to directly evaluate the class bias of different representation spaces and different augmentations of data, accurately predicting and improving performance \textit{without any training}.
%Furthermore, we observe that different encoders will actually change and boost the performance of different classes, and that different augmentations or transformations of data will also induce class dependent spectral effects that can be detected and harnessed for good.
Our empirical results provide strong evidence that spectral imbalance plays a pivotal role in the characteristics of representation space. % pre-trained features.

% divergence in the eigenvalue distributions across classes is predictive of the class gap and which classes will perform better.




%aligning with the theory results.
%We show such phenomena are consistently observed in reality, and can be used to predict the class performance (and imbalance between different classes) without ever training a linear layer. 
%We observe that data augmentation in reality can correct such imbalances, and thus improve class bias.
%Finally, we investigate if it is possible to design augmentations, or correct the existing data augmentations, in order to produce better pre-trained features for better training of the classifier.
%Through the empirical study, we highlight the importance of spectral imbalance in reality, and provide ways to design better augmentations that improve overall performance and class gap.

%\begin{figure}[t]
%\vskip 0.2in
%\begin{center}
%\centerline{\includegraphics[width=\columnwidth]{imgs/overview_placeholder.png}}
%\caption{An image showing how class-wise accuracy is correlated to spectrum property for many classes, with Pearson correlation displayed on right top corner. Would it look bad or something?}
%\label{fig:overview}
%\end{center}
%\vskip -0.2in
%\end{figure}


The major contributions of this work are as follows:
\begin{itemize}
\itemsep0em
    \item We introduce the concept of {\em spectral imbalance} and study how discrepancies in eigenvalues between classes are related to class-dependent generalization.
    \item In Theorem~\ref{thm:main_thm}, we derive \textit{exact} theoretical expressions for the per-class generalization in a high-dimensional linear mixture-model setting. The resultant simulations demonstrate the effect of different spectral imbalances on the per-class performance gap. 
    % \item We characterize the \textit{spectrum-modifying} effect of various common data augmentations and analyze the consequences for the per-class generalization.
    \item Empirically, we show that similar phenomena hold in many pre-trained models. Thus, we design a classwise spectral entropy score, that accurately measures the amount of ``imbalance'' in the representation space.
    % making the spectral property a good evaluation metric on itself to predict the worst performing classes and the amount of ``imbalance'' in different encoders.
    \item Finally, we initiate a study of % the effect of 
    data augmentations under spectral imbalance framework, and provide spectra re-factoring as a method to combine augmentations that improve performance \textit{without any training}.
    % we initiate a study of data manipulation plans, and propose spectra re-factoring
\end{itemize}


==> texts/problemsetup.tex <==
\section{The framework of spectral imbalance}

% Or just show a figure on how severe is this problem.

In this section, we introduce the main idea behind spectral imbalance, and describe its effect on class performance.

\subsection{Setup}
Let $D = (X,y)$ denote a collection of data $X$ with corresponding labels $y$. To characterize the variability and complexity of our data across classes, we will compute the eigenvalue decomposition on a per class basis. This results in a collection of per-class computed eigenvectors and eigenvalues or spectra, that we will denote as $cov(X_i) = V_i D_i V_i^T$ where $V_i$ are the eigenvectors of the covariance of class i and $D_i$ is a diagonal matrix with the eigenvalues for the ith class covariance. We will also denote the jth eigenvalue of class i as $\lambda_{ij}$. See Figure XX for an example of the class-dependent spectra as examples of the different imbalances observed in real data.

\subsection{Class gap}
We next asked if spectral imbalance could be used to predict the class dependent biases in models. 


%Pretrained features themselves are important things, and eigenspectrum is an important tool to study them. Here are why.

%People have checked the class imbalance thing, but they lack proper tools to study it. In this work, we provide a new framework from the perspective of understanding the spectrum.


%The idea of spectral property dates back to XXX. This recently raise more theory attention because its usage on overparameterization regime.



